An Online Self-calibrating Refractive Camera Model with Application to Underwater Odometry

This work presents a camera model for refractive media such as water and its application in underwater visual-inertial odometry. The model is self-calibrating in real-time and is free of known correspondences or calibration targets. It is separable as a distortion model (dependent on refractive index $n$ and radial pixel coordinate) and a virtual pinhole model (as a function of $n$). We derive the self-calibration formulation leveraging epipolar constraints to estimate the refractive index and subsequently correct for distortion. Through experimental studies using an underwater robot integrating cameras and inertial sensing, the model is validated regarding the accurate estimation of the refractive index and its benefits for robust odometry estimation in an extended envelope of conditions. Lastly, we show the transition between media and the estimation of the varying refractive index online, thus allowing computer vision tasks across refractive media.

==> tex/Notes.tex <==
Address SVP camera systems.

Error plot and the distribution and center vertical line, relation with depth.

What makes the camera estimation problem fail.

1) Resolution of the camera, higher is better.
2) FOV of the camera, it must be sufficiently large to allow sinificant refractive distortion.
3) Motion blur, (feature quality and and matching accuracy)
4) Stereo Camera extrinsics


We will also need some good photos of the robot btw in white background to show the sensors etc (if there is space for that).

Short comings of the work:

1) More mature estimation pipeline needed
2) Comparision with kalibr and sub-pixel error validation
3) Incorporate a corrective term for any additional lens distortion.
4) Monocular camera and fundamental matrix
5) Stereo Depth error: Subset of rejrojection error
6) General formulation needed

Learning: 
1) Modelling refractive distortion in sparse features scenario is important.

==> unused/raftmod.tex <==

\subsection{Underwater Depth Prediction}

We develop a stereo dense depth estimation method building upon RAFT-Stereo which itself is a deep architecture for rectified stereo built on top of the optical flow network \ac{raft}. RAFT employs per-pixel features and builds 4D correlation volumes for all pairs of pixels to iteratively update a flow field. RAFT-Stereo further introduced multi-level convolutional \acp{gru} that propagate information across the image more efficiently, while a variant of the method delivers real-time inference. We extend and modify RAFT-Stereo to explicitly consider not only the stereo pair at the current time $t_k$ to offer depth estimation but also the depth estimate during the previous time instance $t_{k-1}$, alongside the odometry estimate connecting the two $\prescript{k-1}{k}{\mathbf{T}} \in SE(3)$. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
\centering
    \includegraphics[width=0.99\columnwidth]{EPS/RAFTStereoRevisited.eps}
\vspace{-2ex}
\caption{TBW. }
\label{fig:raftstereorevisited}
\vspace{-2ex}
\end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



In the original formulation of RAFT-Stereo, the neural network architecture of which is summarized in Figure~\ref{fig:raftstereorevisited}, the stereo camera pair is first rectified. Subsequently, correlation features are derived from the rectified images and organized into a correlation pyramid. Concurrently, "context" image features and an initial hidden state are generated by the content encoder. The disparity field is then set to zero. During each iteration, the current disparity estimate is used by the GRU(s) to sample from the correlation pyramid. These sampled correlation features, along with the initial image features and current hidden states, are utilized by the GRU(s) to update both the hidden state and the disparity.

A key limitation of RAFT-Stereo is that prior information for disparity is not utilized to either improve the consistency of the result or reduce the computational cost. Especially considering the case of static underwater environments (e.g., submerged oil and gas infrastructure) with visual data particularly challenged by the low-light conditions and the presence of turbidity, incorporation of disparity priors can lead to significant improvements. Motivated by this, we revisit RAFT-Stereo and inject history-aware disparity field initialization. Specifically the previous disparity map/depth estimate and the $\prescript{k-1}{k}{\mathbf{T}}$ odometry estimate are utilized to offer a prior in the disparity field of the next iteration. To improve the quality of the disparity prior, the \ac{hpr} operator~\cite{katz2007direct} is first employed. \ac{hpr} identifies the visible points in a point cloud as would be observed from a provided viewpoint. The \ac{hpr} operator is computationally efficient as it avoids surface reconstruction and normal estimation by instead using the convex hull of the transformed point cloud to determine visibility. The predicted disparity map is then used to initialize the respective field in RAFT-Stereo thus leading to computational improvement (including the cost of \ac{hpr} calculations) and image information that allows to overcome challenges introduced by turbidity and other haze-like phenomena. The proposed approach is presented in Figure~\ref{fig:raftstereorevisited}. Among its core benefits for underwater perception is that it demonstrates to be able to be trained purely on synthetic data and transfer with robustness to real-life unerwater data as detailed in Section~\ref{sec:evaluation}. 

\subsection{4D Correlation} 
\subsubsection{RAFT and DEQ}:
\subsubsection{Stereo}
\begin{itemize}
    \item Reprojection error of feature (context) maps to estimate dynamic objects
\end{itemize}
\subsubsection{Monocular}
    \begin{itemize}
        \item Pose-refinement: Pose initialized by Rovio/IMU proprioception, refined by Affine assumption due to small perturbation in close proximity in SE3.
        \item Handling depth near vanishing point
        \item Can it be a factor Graph-based formulation like DeepFactors\cite{Czarnowski2020deepfactors}? (Depending on the scope)
    \end{itemize}
\subsection{Depth Priors}
\subsection{Conformal/Confidence Metric}
\subsubsection{Perception} The uncertainty metric is obtained by Cosine Similarity over warped feature map1 and feature map2 of the correlation volume.

\subsubsection{Localization} The method can estimate the degradation of the robot localization. This is used to estimate the temporal/spatial bounds of the mapping framework. It can further be used to provide conservative control commands during localization degradation.

